Observation of oscillatory relaxation in the Sn-terminated surface of epitaxial rock-salt SnSe $\{111\}$ topological crystalline insulator

Topological crystalline insulators have been recently predicted and observed in rock-salt structure SnSe $\{111\}$ thin films. Previous studies have suggested that the Se-terminated surface of this thin film with hydrogen passivation, has a reduced surface energy and is thus a preferred configuration. In this paper, synchrotron-based angle-resolved photoemission spectroscopy, along with density functional theory calculations, are used to demonstrate conclusively that a rock-salt SnSe $\{111\}$ thin film epitaxially-grown on \ce{Bi2Se3} has a stable Sn-terminated surface. These observations are supported by low energy electron diffraction (LEED) intensity-voltage measurements and dynamical LEED calculations, which further show that the Sn-terminated SnSe $\{111\}$ thin film has undergone a surface structural relaxation of the interlayer spacing between the Sn and Se atomic planes. In sharp contrast to the Se-terminated counterpart, the observed Dirac surface state in the Sn-terminated SnSe $\{111\}$ thin film is shown to yield a high Fermi velocity, $0.50\times10^6$m/s, which suggests a potential mechanism of engineering the Dirac surface state of topological materials by tuning the surface configuration.

==> Paper In LaTeX/author_list.tex <==
% Author list

\author{Wencan Jin}
\altaffiliation{These authors contribute equally to this work.}
\affiliation{Columbia University, New York, New York 10027, USA}

\author{Suresh Vishwanath} 
\altaffiliation{These authors contribute equally to this work.} 
\affiliation{Cornell University, Ithaca, New York 14853, USA}

\author{Jianpeng Liu} 
\affiliation{Kavli Institute for Theoretical Physics, University of California, Santa Barbara, California 93106, USA }

\author{Lingyuan Kong} 
\affiliation{Beijing National Laboratory for Condensed Matter Physics, and Institute of Physics, Chinese Academy of Sciences, Beijing 100190, China}

\author{Rui Lou} 
\affiliation{Department of Physics, Renmin University of China, Beijing 100872, China}

\author{Zhongwei Dai} 
\affiliation{University of New Hampshire, Durham, NH 03824, USA}

\author{Jerzy T. Sadowski} 
\affiliation{Center for Functional Nanomaterials, Brookhaven National Laboratory, Upton, New York 11973, USA}

\author{Xinyu Liu} 
\affiliation{University of Notre Dame, Notre Dame, Indiana 46556, USA}

\author{Huai-Hsun Lien} 
\affiliation{Cornell University, Ithaca, New York 14853, USA}

\author{Alexander Chaney} 
\affiliation{Cornell University, Ithaca, New York 14853, USA}

\author{Yimo Han}
\affiliation{Cornell University, Ithaca, New York 14853, USA}

\author{Micheal Cao}
\affiliation{Cornell University, Ithaca, New York 14853, USA}

\author{Junzhang Ma} 
\affiliation{Beijing National Laboratory for Condensed Matter Physics, and Institute of Physics, Chinese Academy of Sciences, Beijing 100190, China}

\author{Tian Qian} 
\affiliation{Beijing National Laboratory for Condensed Matter Physics, and Institute of Physics, Chinese Academy of Sciences, Beijing 100190, China}

\author{Jerry I. Dadap} 
\affiliation{Columbia University, New York, New York 10027, USA}

\author{Shancai Wang} 
\affiliation{Department of Physics, Renmin University of China, Beijing 100872, China}

\author{Malgorzata Dobrowolska}
\affiliation{University of Notre Dame, Notre Dame, Indiana 46556, USA}

\author{Jacek Furdyna} 
\affiliation{University of Notre Dame, Notre Dame, Indiana 46556, USA}

\author{David A. Muller}
\affiliation{Cornell University, Ithaca, New York 14853, USA}

\author{Karsten Pohl} 
\affiliation{University of New Hampshire, Durham, NH 03824, USA}

\author{Hong Ding} 
\affiliation{Beijing National Laboratory for Condensed Matter Physics, and Institute of Physics, Chinese Academy of Sciences, Beijing 100190, China}

\author{Huili Grace Xing}
\email{grace.xing@cornell.edu} 
\affiliation{Cornell University, Ithaca, New York 14853, USA}
\affiliation{University of Notre Dame, Notre Dame, Indiana 46556, USA} 

\author{Richard M. Osgood, Jr} 
\email{osgood@columbia.edu}
\affiliation{Columbia University, New York, New York 10027, USA}
